Stress-controlled medium-amplitude oscillatory shear (MAOStress) of PVA-Borax

We report the first-ever complete measurement of MAOStress material functions, which reveal that stress can be more fundamental than strain or strain rate for understanding linearity limits as a function of Deborah number. The material used is a canonical viscoelastic liquid with a single dominant relaxation time: Polyvinyl alcohol (PVA) polymer solution crosslinked with tetrahydroborate (Borax) solution. We outline experimental limit lines and their dependence on geometry and test conditions. These MAOStress measurements enable us to observe the frequency dependence of the weakly nonlinear deviation as a function of stress amplitude. The observed features of MAOStress material functions are distinctly simpler than MAOStrain, where the frequency dependence is much more dramatic. The strain-stiffening transient network model (SSTNM) was used to derive a model-informed normalization of the nonlinear material functions that accounts for their scaling with the linear material properties. Moreover, we compare the frequency-dependence of the critical stress, strain, and strain-rate for the linearity limit, which are rigorously computed from the MAOStress and MAOStrain material functions. While critical strain and strain-rate change by orders of magnitude throughout the Deborah number range, the critical stress changes by a factor of about two, showing that stress is a more fundamental measure of nonlinearity strength. This work extends the experimental accessibility of the weakly nonlinear regime to stress-controlled instruments and deformations, which reveal material physics beyond linear viscoelasticity but at conditions that are accessible to theory and detailed simulation.

==> Text/z-manuscript.tex <==

\section{Introduction}
Measuring the nonlinear viscoelastic response of complex fluids provides valuable insights into their constitutive behavior and underlying physics. One technique for studying the nonlinear response is large-amplitude oscillatory shear (LAOS)\cite{Hyun2011ALAOS,Giacomin1993Large-amplitudeShear,Wilhelm2002FourierTransformRheology,Ewoldt2008NewShear}, which has been used to study a wide range of complex materials\cite{Komatsu1973NonlinearEmulsions,Neidhofer2004DistinguishingRheology,KateGurnon2012LargeMicelles,Dealy2013MeltIndustry,Randall2014Linear-nonlinearPolymers,Joyner2021NonlinearQuality}. However, this technique can be hindered by noisy data, sample issues, and difficulty in relating the results to models. Weakly nonlinear methods, such as medium-amplitude oscillatory shear (MAOS)\cite{Hyun2009EstablishingSystems,Ewoldt2013Low-dimensionalViscoelasticity, KateGurnon2012LargeMicelles,Kumar2016IntrinsicSuspensions,Singh2017Frequency-sweepMAOS,Bharadwaj2017AShear,Carey-DeLaTorre2018First-harmonicMAOS,Natalia2020QuestioningExpansions} and medium amplitude superposition (MAPS)\cite{Lennon2020MediumExamples,Shanbhag2022KramersKronigImplications}, offer a sweet spot between small-amplitude oscillatory shear (SAOS) and LAOS probing a regime with rich detail that is theoretically tractable.

\begin{figure}[h!]
 \includegraphics{Figures/Chapter3/IntroFigure.pdf}%
 \caption{MAOStrain vs MAOStress. Linear moduli and compliances are interchangeable but exhibit different features. Nonlinear MAOStrain material functions ($[e_1]$, $[v_1]$, $[e_3]$, and $[v_3]$) were measured before\cite{Bharadwaj2017AShear}, but we repeat here for consistency (Appendix C). The critical strain for nonlinearity can be calculated from the MAOStrain material functions(Eq. 5 in Ewoldt and Bharadwaj\cite{Ewoldt2013Low-dimensionalViscoelasticity}, with $\epsilon=10\%$). This work aims to measure the dependence of MAOStress material functions on frequency for the first time, revealing how the critical stress to nonlinearity depends on frequency. The data used here is for the 2.75\%PVA/1.25\%Borax sample investigated in this work. \label{fig:3intro}}%
 \end{figure}
 
MAOS probes the gradual deviation from linearity in an oscillatory test. For example, applying a sinusoidal strain input $\gamma(t)=\gamma_0\sin \omega t$ in strain-controlled MAOS (MAOStrain) results in a stress response that can be written as 

\begin{align}
\sigma (t)=\gamma_0\left( \right.& \left.G^{\prime}\sin\omega t+G^{\prime\prime}\cos \omega t \right) \nonumber\\
+\gamma_0^3& \left( [e_1]\sin \omega t+[v_1]\omega \cos \omega t\right.  \\
-&\left. [e_3]\sin 3 \omega t+[v_3] \omega \cos 3\omega t\right) ,\nonumber
\end{align}
where $[e_1]$, $[v_1]$, $[e_3]$, and $[v_3]$ are the frequency-dependent intrinsic Chebyshev nonlinearities defined by Ewoldt et al. \cite{Ewoldt2013Low-dimensionalViscoelasticity}. Measuring these material functions provides more information about the material, quantifying changes in the nonlinear material response as a function of frequency (e.g., Figure \ref{fig:3intro}). This regime is also accessible to analytical model solutions\cite{Bharadwaj2015ConstitutiveShear,Saengow2017ExactStress,Martinetti2019Time-strainShearb,Bharadwaj2017AShear,Song2020EvaluatingSolutions,Ramlawi2020TheModel}, which allows for material-property inference using information from both the linear and nonlinear material response\cite{Singh2022OnCertainty}. MAOStrain, for instance, has been used to solve a 70-year-long debate in the literature about the origin of strain-stiffening in transient polymer networks\cite{Martinetti2018InferringNetworkb}. Moreover, the MAOS material functions can be used to calculate the linearity limits of viscoelastic materials as a function of frequency through quantifying the absolute strength of the nonlinear deviation compared to the linear term. The linearity limits can be used to describe the regime boundary on a Pipkin map\cite{Pipkin1986LecturesTheory,Dealy1999MeltProcessing,Ewoldt2013Low-dimensionalViscoelasticity,Giacomin2011Large-amplitudeModel} to separate linear and nonlinear regimes

The MAOS approach to compute linearity limits in an oscillatory test is more rigorous than using the total deviation in the first harmonics. Since the nonlinear transition is gradual, linearity limits are typically defined as the forcing amplitude (stress, strain, or strain rate) at which the deviation from the linear plateau of a nonlinear material function exceeds a subjective threshold $\epsilon$ (e.g. $\frac{|G_1^{\prime}(\gamma_0)-G^{\prime}|}{G^{\prime}}>\epsilon$)\cite{Pearson1982BehaviorFields}. The MAOS material functions quantify this gradual transition\cite{Ewoldt2013Low-dimensionalViscoelasticity} (e.g. $G_1^{\prime}=G^{\prime}+[e_1]\gamma_0^2+...$ for small enough amplitudes), can be used to define a critical forcing amplitude for an arbitrary threshold (e.g. $\frac{\gamma_{0,crit}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{G^{\prime}(\omega)}{[e_1](\omega)}}$ and $\dot{\gamma_{0,crit}}=\omega\gamma_{0,crit}$), as shown in Figure \ref{fig:3intro}. The benefit of using the MAOS definition instead of the total deviation is that the total deviation may not be measurable for small thresholds, unlike the MAOS deviation that is quantifiable at any amplitude if the material function is measured. 

Nonlinear oscillatory measurements can be conducted in both strain-control and stress-control modes. While most of the LAOS measurements in the literature are strain-controlled (LAOStrain), many works used LAOStress (stress-controlled LAOS) to explore the nonlinear response of materials\cite{Dimitriou2013DescribingLAOStress,Pineiro-Lago2023LargePDO}. Stress-controlled results can be connected directly to many practical applications, such as gravity and pressure-driven flows. For certain materials, such as yield-stress fluids, stress-controlled oscillations allow for direct probing of the yielding transition and can add to the understanding derived from LAOStrain measurements. Moreover, Lauger and Stettin showed that LAOStrain and LAOStress probe a different material behavior, where significant differences in the Lissajous stress-strain curves were observed for Xantham gum\cite{Lauger2010DifferencesFluids}. Hence, a better understanding of stress-controlled nonlinear measurements will increase the accessibility of MAOS measurements. 

MAOStress has been theoretically anticipated since at least 2013 but has yet to be experimentally measured. The theory for Stress-controlled MAOS (MAOStress) was developed by Ewoldt and Bharadwaj in 2013. For a co-sinusoidal stress input $\sigma (t)=\sigma_0\cos \omega t$, the strain in the weakly nonlinear regime can be expanded as 
\begin{align}
\gamma(t)=\bar{\gamma}(\omega,\sigma_0)+\sigma_0  &\left(J^{\prime}\cos\omega t+J^{\prime\prime}\sin \omega t\right)\nonumber\\
+\sigma_0^3&\left( [c_1]\cos \omega t+\frac{[f_1]}{\omega} \sin \omega t\right.\\
+&\left.[c_3]\cos 3 \omega t+\frac{[f_3]}{3\omega}\sin 3\omega t\right),\nonumber
\end{align}
where $[c_1]$, $[f_1]$, $[c_3]$, and $[f_3]$ are the frequency-dependent intrinsic Chebyshev nonlinear compliances and fluidities and $\bar{\gamma}(\omega,\sigma_0)$ is the baseline strain, as defined by Ewoldt et al. \cite{Ewoldt2013Low-dimensionalViscoelasticity}. Similar to MAOStrain, a critical stress amplitude $\sigma_{0,crit}$ can also be defined based on the measured MAOS material functions. While many MAOStrain measurements have been reported since, no frequency-dependent MAOStress material functions have been previously reported.  

 In this work, we make the first-ever MAOStress measurement to test the weakly nonlinear response of PVA-Borax, including $\gamma_{0,crit}$, $\dot{\gamma}_{0,crit}$, and $\sigma_{0,crit}$. PVA-Borax has been well-studied using MAOStrain\cite{Bharadwaj2017AShear,Martinetti2018InferringNetworkb}, making it a model material to compare the two protocols. In the linear regime, stress and strain-control protocols are interchangeable, but the stress-controlled perspective can still show a much simpler response (Figure 1). Therefore, we are interested in examining how the material response signatures differ between these two methods. With the four MAOStrian and MAOstress material functions, one can identify the frequency-dependent limits of the linear viscoelastic approximation (i.e. the strength of nonlinearity, which can be reinterpreted as a critical forcing strength where nonlinearity is 'significant' in terms of critical strain amplitude, or strain rate amplitude, or stress amplitude). We compare the frequency dependence of critical stress, strain, and strain rate for the emergence of nonlinearity. We show that stress is a more universal measure of nonlinearity strength, where the critical stress to enter the nonlinear regime varies minimally with frequency compared to strain and strain rate.
 
This work is organized as follows: First, we introduce the material preparation protocol, the theoretical framework for MAOStress, and the experimental procedure that was followed. Section 3 presents the experimental measurement of the MAOStress material functions, where the frequency dependence of the weakly nonlinear response is thoroughly analyzed, in addition to analysis of the scaling of the nonlinear material functions with linear properties. Section 4 discusses the implications of the results on the frequency dependence of the stress at the onset of the nonlinear regime, showing how Pipkin map limit lines can be affected by the choice of strain, strain rate, or stress as the measure of nonlinearity strength.


\label{Sec: Intro}

\section{Materials and Methods}

 \begin{figure}[h!]
 \includegraphics{Figures/Chapter3/Fig2MaterialsAndMethods.pdf}%
 \caption{Materials and methods. (a) PVA-Borax is a transient polymer network with $\tau ~ 0.4$s, allowing it to (b) bounce upon impact (short times) while creeping under its weight at long times as assessed by protorheology\cite{HossainProtorheology}. (c) Cone-plate geometry was used on a stress-controlled rheometer to impose a stress cosinusoidal input signal. The directly measureable quantities are torque $M(t)$ and angular displacement $\theta(t)$, which are proportional to stress ($\sigma(t)=\frac{2}{\pi R^3}M(t)$) and strain ($\gamma(t)=\frac{1}{\tan \alpha}\theta(t)$) respectively, where $R$ and $\alpha$ are the radius and angle of the cone, respectively. (d) The measured strain waveform will deviate from the ideal sinusoidal shape at increasing stress amplitude $\sigma_0$. Discrete Fourier transform will be used to identify the strain harmonics $\{\gamma_1^{\prime},\gamma_1^{\prime\prime},\gamma_3^{\prime},\gamma_3^{\prime\prime}\}$  (Eq. \ref{eq:3 Fourier expansion}) at every amplitude, which are fit to Eq. \ref{eq:3 harmnonics expansion} to find the MAOStress material functions at each frequency.  \label{fig:3Materials and Methods}}%
 \end{figure}
 
\subsection{Mathematical Framework}
%Objectives: Clearly outline the assumptions made in MAOS. Make the math simple and tractable. 
The strain response to an oscillatory shear stress deformation $\sigma (t)=\sigma_0\cos \omega t$ can be written as a Fourier expansion in terms of the odd harmonics\cite{Ewoldt2013DefiningShear,Hyun2011ALAOS}, in addition to a baseline strain $\bar{\gamma}$
\begin{equation}
\label{eq:3 Fourier expansion}
    \gamma(t;\sigma_0,\omega)=\bar{\gamma}(\sigma_0,\omega)+\sum_{n,\mathrm{odd}} \gamma_n^{\prime}(\sigma_0,\omega)\cos n\omega t+\gamma_n^{\prime\prime}(\sigma_0,\omega)\sin n\omega t
\end{equation}
where $\gamma_n^{\prime}$ and $\gamma_n^{\prime\prime}$ are the $\mathrm{n^{th}}$ elastic and viscous strain harmonics, respectively. For sufficiently small amplitudes, the strain behaves linearly, where only the first harmonics, $\gamma_1^{\prime} $ and $\gamma_1^{\prime\prime}$, are required to describe the response, and these harmonics scale linearly with stress amplitude. In this limit of $\sigma_0 \to 0$, referred to as small-amplitude oscillatory shear (SAOS), the stress-independent linear elastic compliance $J^{\prime}(\omega)=\gamma_1^{\prime}/\sigma_0 $ and linear viscous compliance $J^{\prime\prime}(\omega)=\gamma_1^{\prime\prime}/\sigma_0 $ capture the frequency-dependence of the viscoelastic behavior. However, as the amplitude increases, the linearity with stress amplitude is broken by the emergence of higher harmonics and changes to the now amplitude-dependent first-harmonics. One common assumption is that these harmonics can be expanded as a function of the stress amplitude $\sigma_0$ using a Taylor series, which applies to many materials. Nevertheless, some materials have shown non-integer power expansions\cite{Natalia2020QuestioningExpansions, Natalia2019RheologicalShear}, which can be predicted from physical models as well. However, since previous experimental observations of PVA-Borax showed that a Taylor-series expansion works for that material, we expand the strain harmonics as integer powers. 
In the first deviation from linearity, only the first and third harmonics are present\cite{Ewoldt2013Low-dimensionalViscoelasticity}, and the first and third strain harmonics up to the first deviation are expanded as
\begin{subequations}
\label{eq:3 harmnonics expansion}
\begin{eqnarray}
\gamma_1^{\prime}(\sigma_0,\omega)=J^{\prime}\sigma_0 + [c_1]\sigma_0^3+ \mathcal{O}(\sigma_0^5)\\
\gamma_1^{\prime\prime}(\sigma_0,\omega)=J^{\prime\prime}\sigma_0 + \frac{[f_1]}{\omega}\sigma_0^3+ \mathcal{O}(\sigma_0^5)\\
\gamma_3^{\prime}(\sigma_0,\omega)= [c_3]\sigma_0^3+ \mathcal{O}(\sigma_0^5)\\
\gamma_3^{\prime\prime}(\sigma_0,\omega)= \frac{[f_3]}{3\omega}\sigma_0^3+ \mathcal{O}(\sigma_0^5)
\end{eqnarray}
\end{subequations}
The first-harmonic intrinsic nonlinearities, $[c_1]$ and $[f_1]$, quantify the degree to which changes in the first harmonics occur as the stress amplitude increases, causing intracycle changes in the material response. The sign of these material functions determines whether softening, stiffening, thinning, or thickening occur as amplitude increases. The third harmonic intrinsic nonlinearities $[c_3]$ and $[f_3]$ quantify the first-order growth of the third harmonics of strain, causing increased distortion in the Lissajous curves.

\subsection{Experimental Protocol}
The stress-controlled oscillatory amplitude sweeps were conducted on the MCR 702 twin-drive rotational rheometer. We used a cone and plate geometry ($d = 25 \mathrm{mm}$, $\alpha=4^{\circ}$) to ensure homogeneous stress and strain distribution within the sample. The temperature was controlled using a bottom Peltier plate at $25^{\circ}\mathrm{C}$. After loading, the sample was coated with a thin layer of silicone oil at the edge of the gap to prevent water evaporation from the sample. 

The material functions were extracted at every frequency by fitting the stress amplitude sweeps to Eqs. \ref{eq:3 harmnonics expansion}a-d. The maximum stress amplitude tested has to be high enough to resolve the MAOS regime experimentally. However, it is preferred to avoid high stresses beyond the MAOS regime and may cause irreversible changes to the material. This allows us to use the same sample to test multiple frequencies, simplifying the experimental protocol. Hence, several pretests were run to find the maximum stress amplitude we can reach at every frequency without causing irreversible change by comparing the linear viscoelastic frequency sweep before and after the sweep. This maximum amplitude and the minimum amplitude required to resolve the MAOS regime experimentally vary as a function of frequency. Therefore a different stress range is set at each frequency. Moreover, the time required to complete the sweeps at the low frequency can exceed 24 hours, which puts the sample at risk of evaporation despite the use of silicone oil. For this reason, multiple loadings were used to test the entire frequency range.

The full frequency range ($\omega=[0.1-100] \mathrm{rad/s}$)  was tested in three different loadings. We used $\sigma_0=[1-300]$Pa for $\omega=[0.1-1] \mathrm{rad/s}$, $\sigma_0=[1-500]$Pa for $\omega=[1.0-10.0] \mathrm{rad/s}$, and $\sigma_0=[1-1000]$Pa for $\omega=[10.0-100.0] \mathrm{rad/s}$. Moreover, we used 50 points per decade of stress amplitude $\sigma_0$ to get good resolution and to ensure that the steps in stress amplitude are small, such that the equilibration time from one amplitude to the other is low. 
 \begin{figure}[h!]
 \includegraphics[width=\textwidth]{Figures/Chapter3/Figure2vB.pdf}%
 \caption{(a) Amplitude sweep of first-harmonic compliances $J_1^{\prime}$ and $J_1^{\prime\prime}$ showing the stiffening and thickening occurring in PVA-Borax at $\omega=5$ rad/s in the range of stress amplitude tested. (b) The weakly nonlinear deviation of $J_1^{\prime}$ can be isolated and fit after subtracting the linear term $J^{\prime}\sigma_0$. The noise floor at around $~10^{-5}-10^{-6}$ is due to instrument limitations and ambient noise.}
 \label{fig:3Sweep Illustration}
 \end{figure}


A custom Python code is used to process the stress and strain waveforms at every amplitude and frequency using a discrete Fourier transform to extract the strain harmonics $\{\gamma_1^{\prime}, \;\gamma_1^{\prime\prime},\; \gamma_3^{\prime}, \;\gamma_3^{\prime\prime}\}(\sigma_0,\omega)$. The harmonic sweeps of the first-harmonic compliances ($J_1^{\prime}$ and $J_1^{\prime\prime}$) can be used to identify the overall response of the material to the applied stress. An amplitude sweep for PVA-Borax is shown in Figure \ref{fig:3Sweep Illustration} an at $\omega=5$ rad/s. The decrease in compliance at increasing amplitudes highlights the stiffening and thickening nature of these networks. While the linear compliances can be extracted from the first-harmonic compliances sweep, the intrinsic nonlinear coefficients are computed by isolating the nonlinear deviations as shown in Figure \ref{fig:3Sweep Illustration}b. The linear term can be subtracted from the elastic first-harmonic in Eq. \ref{eq:3 harmnonics expansion}a to isolate the weakly nonlinear term. At every frequency, the four weakly nonlinear deviations ($\{\gamma_1^{\prime}, \;\gamma_1^{\prime\prime},\; \gamma_3^{\prime}, \;\gamma_3^{\prime\prime}\}(\sigma_0,\omega)$) are fit to Eq. \ref{eq:3 harmnonics expansion} to extract the MAOStress material functions $J^{\prime}$, $J^{\prime\prime}$, $[c_1]$, $[c_3]$, $[f_1]$, and $[f_3]$. The range of the fit was restricted to the experimental MAOS regime, which is lower bounded by the noise floor and upper bounded by the higher order terms (>$\sigma_0^3$). The fits and the corresponding ranges are documented in the Supplementary Information (SI). 

Experimental limits\cite{Ewoldt2015ExperimentalData} for the measured harmonics and compliances are useful to determine the accessible experimental window. For the strain harmonics, the window is set by the low torque limit $M_{\mathrm{min}}$
\begin{equation}
    {
    \label{eq:3Mmin}
 \sigma_{\mathrm{min}}=F_\sigma M_{\mathrm{min}}
}
\end{equation}
high torque limit $M_{\mathrm{max}}$
\begin{equation}
{
\label{eq:3Mmax}
     \sigma_{\mathrm{max}}=F_\sigma M_{\mathrm{max}}
}
\end{equation}
and minimum displacement limit $\theta_{\mathrm{min}}$ \begin{equation}
{\label{eq:3thetaMin}
\gamma_{\mathrm{min}}=F_{\gamma}\theta_{\mathrm{min}} }
\end{equation}of the instrument. For a cone and plate geometry, $F_{\sigma}=\frac{2}{\pi R^3}$ and $F_{\gamma}=\frac{1}{\tan \alpha}$, where $R$ is the radius of the geometry and $\alpha$ is the degree of the cone. The minimum measurable compliance can be inferred from the minimum strain as $J_{\mathrm{min}}=\gamma_{\mathrm{min}}/\sigma_0$. Figure \ref{fig:3Experimental limits} demonstrates how the experimental limits can be used to identify the theoretically accessible experimental window of the instrument, e.g., based on the manufacturer specifications shown in Table \ref{tab:MCRspecs}. The predicted low-displacement limit is only an order of magnitude higher than the measured limit of $\gamma_{\mathrm{min}}~10^{-5}$. Moreover, the weakly nonlinear deviation characterized by the slope of 3 for the third harmonics in Figure \ref{fig:3Experimental limits} can be significantly below the high-torque limit of the instrument. Despite that, the predicted low-torque limit is $\sigma_{\mathrm{min}}~10^{-2}$ Pa, and the raw waveforms were found to be noisy below $\sigma_0=10$ Pa. Therefore, the low-stress limit from Eq. \ref{eq:3Mmin} may not directly translate to the stress amplitude that can be measured. One possible explanation is that the torque is controlled in steps much smaller than the stress amplitude during an oscillatory test. For example, for the 512 points per cycle used, the minimum stress change between successive points can be found at the peak of the oscillatory wave. It can be estimated as $\frac{\Delta \sigma_{min}}{\sigma_0} =|\cos(0)-\cos(\Delta t\omega)|$, where $\Delta t\omega=2\pi/512$ is for a fixed time interval between points. Therefore the minimum stress amplitude that can be controlled should be $\sigma_{0,\mathrm{min}}=\frac{\Delta \sigma_{min}}{1-\cos(2\pi/512)}\approx \frac{F_{\sigma}M_{\max}}{7*10^{-5}}=4$Pa for the geometry used in this work. This value provides a good starting point for experimental design, where the difference between the predicted (4 Pa) and actual (around 10 Pa from Figure \ref{fig:3Experimental limits}) low-stress limit is around a factor of 2 and can be due to ambient noise.  

\begin{figure}[h!]
\centering
 \includegraphics{Figures/Chapter3/FigExptlLimits.pdf}%
 \caption{Experimental limit lines for stress amplitude sweeps. Limit lines for low-torque (Eq. \ref{eq:3Mmin}), high-torque (Eq. \ref{eq:3Mmax}), and minimum angular displacement (Eq.\ref{eq:3thetaMin}) plotted for 25mm cone-plat e using the instrument specs in Table \ref{tab:table1}. PVA-Borax data collected at 1 rad/s shows that the true limit line is about one order of magnitude higher than the theoretical limit line. \label{fig:3Experimental limits}}%
 \end{figure}

 
\begin{table}
\centering
\caption{\label{tab:MCRspecs}MCR 702 manufacturer instrument specification.}
\begin{tabular}{ >{\raggedright\arraybackslash}p{0.1\linewidth}  >{\raggedright\arraybackslash}p{0.1\linewidth}>{\raggedright\arraybackslash}p{0.1\linewidth} }
 $M_{\mathrm{min}}$ & $M_{\mathrm{max}}$&
$\theta_{\mathrm{min}}$\\
\hline
0.5nN.m & 230mN.m & 50nrad \\
\end{tabular}

\end{table}
\subsection{Material Preparation}
The PVA-Borax sample in this work contains 2.75 wt\% Polyvinyl alcohol (PVA) aqueous solution physically crosslinked with 1.25 wt\% Sodium tetraborate (Borax). The concentration was selected following the work of Bharadwaj et al.\cite{Bharadwaj2017AShear}. The sample was prepared as follows: 4wt\% PVA (Sigma-Aldrich, 99\% hydrolyzed, Mw = 85,000-110,000) was dissolved in DI water at $80^\circ \mathrm{C}$ overnight until a homogeneous transparent solution was obtained. Similarly, 4wt\% Borax (Sigma-Aldrich) solution was prepared by dissolving Borax in DI water. After the stock solutions cooled down to room temperature, the two solutions were mixed (27.5 PVA:12.5 Borax by solution mass) to prepare 2.75wt\% PVA- 1.25wt\% Borax solution. Air bubbles trapped during the mixing were removed by centrifuging.

Protorheology\cite{HossainProtorheology}, shown in Figure 2(b), reveals that PVA-Borax behaves as a viscoelastic liquid with a finite flow viscosity $\eta_{\infty}$ and an observable relaxation time $\tau_C$. Using the viscous gravity current experiment, we observe that the material exhibits flow over extended periods and that the viscosity can be estimated as $\eta=0.0195\rho g \Delta t\frac{h_2^3(3R_2^2+h_2^2)^3}{R_2^8-R_1^8}$ where $\rho$ is density, $\Delta t$ is elapsed time, $h_2$ is final height and $R_1$, $R_2$ are the initial and final radius, respectively. From Figure 2(b), we have $R_1$ = 1.6 cm, $R_2$ = 2.4 cm and $h_2$ = 1.1 cm and using $\rho$ = 103 kg/m3 and g = 9.8 N/kg, we obtained $\eta \approx 4500 \mathrm{Pa.s}$ at a characteristic stress of $\sigma_{grav} \approx 220 Pa$. The observation time of 300s (corresponding to $\omega=2\times 10^{-2}$  rad/s) suggests that the material is entering a terminal regime where $G^{\prime\prime} = \eta.\omega=95$ Pa is anticipated. The bounce test in Fig. 2(b) shows that the material has elasticity at short times and $tan\delta$ can be estimated from $\tan \delta=\frac{1}{\pi}ln(\frac{1}{f})$, where $f=h_{reb}/h_{drop}$ is the recovered height fraction.  From Figure 2(b) we have f = 0.38 which gives $tan\delta \approx0.3$ (corresponding to $\omega=\pi/\Delta t \approx157$ rad/s where $\Delta t \approx 20$ ms) at a characteristic stress of $\sigma\approx210 Pa$. These experiments bound the time scale to be >20 ms and less than 15s. The protorheology observations do not indicate the nature of nonlinearity, for which more accurate rheometry will be used. 
\newpage
\section{Results}
\begin{figure}[H]
{ \includegraphics[width=\textwidth]{Figures/Chapter3/figAmpSweeps.pdf}%
 \caption{Stress amplitude sweeps of (a) elatsic $J_1^{\prime}$ and (b) viscous $J_1^{\prime\prime}$ first-harmonic compliances at $\omega={0.1, 1, 10, 39.8}$rad/s.  Dashed lines show $J^{\prime}$ and $J^{\prime\prime}$ values obtained from the fits. The corresponding growth of the elastic (c) and viscous (d) first-harmonic deviations are with a power-law of 3 (Eq.\ref{eq:3 harmnonics expansion}). Similarly, elastic (e) and viscous (f) third harmonics' leading order term is fit with a power-law of 3. Closed symbols represent positive values, and open symbols represent negative values. Similar plots for all frequencies are shown in the supplementary information}%
  \label{fig:3AmpSweep}}
 \end{figure}

Stress amplitude sweeps of PVA-Borax were conducted in the frequency range of [0.1-100 rad/s], and the resulting first and third strain harmonics are shown in Figure \ref{fig:3AmpSweep} for frequencies of $\omega=[0.1,1,10,39.8]$ rad/s. The first-harmonic compliances exhibited a typical linear regime plateau, followed by a slight decrease due to the stress-stiffening nature of the material. The slight decrease in compliance led to orders of magnitude growth in the weakly nonlinear deviations of the first harmonics. These deviations were computed by subtracting the linear contributions, calculated as $J^{\prime}\sigma_0$ and $J^{\prime\prime}\sigma_0$ for the elastic and viscous first harmonics. The fit lines in Figures \ref{fig:3AmpSweep}(c)-(f) demonstrate that the first and third-harmonic deviations grew closely to $\sigma_0^3$, consistent with the theory and measurements of the weakly nonlinear deviations in MAOStrain. The material functions associated with the fit lines were extracted as described in the methods section, and the fits for all the frequencies are shown in the SI. The deviations grow after a certain amplitude where the signal exceeds the noise floor. This noise was above the value predicted from the instrument limits using Equation 2.

Furthermore, the noise floor increased with the experimental frequency. These observations can be explained by external factors, such as ambient noise, instrument state, and sample loading, that are difficult to predict a priori and are not accounted for by instrument calibration. Nonetheless, the minimum observable strain amplitude achieved was remarkably low ($<10^{-5}$) and was enough to extract the MAOStress material functions.

The frequency-dependent behavior of the extracted linear elastic compliance $J^{\prime}$ and viscous fluidity $\phi^{\prime}=J^{\prime\prime}*\omega$ is presented in Figure \ref{fig:3SAOSSweep}. The LVE behavior of PVA-Borax deviates from a single-mode Maxwell model due to its distribution of relaxation times, which was captured by a continuous Lognormal distribution (Appendix A). The relaxation time $\tau_0=0.402$s, dispersity index$D=2.54$ and elastic compliance $J_0=\frac{1}{G_0}=0.9\times 10^{-3}\mathrm{Pa^{-1}}$ were extracted from the moments of the distribution\cite{Martinetti2018ContinuousShear}. The viscous compliance $J^{\prime\prime}$ at the high frequencies ($\omega>60$ rad/s) is noisy, because it is the sub-dominant compliance component ($\tan \delta<0.1$)\cite{Singh2019OnRepresentation}. This caused the fits to have an unsatisfactory adjusted coefficient of determination $R^2_{adj}$ (documented in the SI) associated with the goodness of fit, and therefore the corresponding material functions are omitted from the results.

The frequency dependence of MAOStress material functions is reported in Figure \ref{fig:3MAOStrain}(a-d). The sign of the material functions is indicated by whether the symbol is filled (positive) or not (negative). The negative sign of the first-harmonic material functions $[c_1]$ and $[f_1]$ shows that PVA-Borax stiffens and thickens with increasing stress across all the tested frequencies. The value of the normalized material function can be used to compare to models or other material formulations to fit model parameters or establish benchmarks for desired nonlinearity in different applications. The material functions are normalized to represent the relative strength of the nonlinearity to the linear component, which will be further discussed below. The magnitude of $[c_1]$ decreases as a function of frequency, which shows that the stress-stiffening nonlinearity decreases in the elastic limit (high frequencies).
On the other hand, the viscous nonlinearity is constant at the lower frequencies until $\omega=10 \;\mathrm{rad/s}$, at which point a sharp decrease is observed, showing that the viscous thickening is weak in the elastic limit. Another reason behind this drop could be the difficulty of measurement because the viscous component is subdominant, as discussed above. The same material's MAOStrain results are unaffected at those frequencies (Figure \ref{fig:3MAOStrain}), which can be due to optimized control for oscillatory strain in commercial instruments compared to oscillatory stress. 

Third-harmonics are associated with the distortion of Lissajous curves\cite{Ewoldt2008,Ewoldt2013Low-dimensionalViscoelasticity,Pineiro-Lago2023LargePDO}. The sign of the third-harmonics determines the concavity of the stress-strain Lissajous curves. A negative value of $[c_3]$ and $[f_3]$ means that within an oscillation cycle in the weakly nonlinear limit, the elastic and viscous compliance of the material decreases with stress and that the degree at which this decrease occurs increases with stress amplitude (material is stiffer/thicker at higher stress). Combining this intracycle change with the observed stiffening and thickening at increasing amplitudes, we can deduce that the stiffening occurs due to increased stress and not stress rates(Check Figure 7 in Ewoldt and Bharadwaj\cite{Ewoldt2013Low-dimensionalViscoelasticity}). The positive sign of $c_3$ for $\omega>10 \mathrm{rad/s}$ suggests that the stiffening is happening in that range due to increasing stress rates and not stress. The ratio of the  $[c_3]$ to $[c_1]$ and $[f_3]$ to $[f_1]$ is comparable to  model prediction from the SSTNM model ($\approx 0.3$) as derived in the SI. More about the mathematics behind this interpretation can be found in Ewoldt 2013\cite{Ewoldt2013Low-dimensionalViscoelasticity}.


\begin{figure}[h!]
 \includegraphics{Figures/Chapter3/SAOSSweepCPPresent-radj.pdf}%
 \caption{LVE material functions: (a) elastic compliance $J^{\prime}$ and (b) viscous fluidity $\phi^{\prime}$ show a small change as a function of frequency (both will be constant for single-mode Maxwell model). The lognormal spectrum fit (SI) is used to compute the elastic plateau modulus $G_N^0=1102$ Pa and average timescale $\tau_0=0.402$ s  from which the elastic compliance $J_0=\frac{1}{G_N^0}$ and infinite time fluidity $\phi_0=\frac{1}{G_N^0\tau_0}$ are computed.}%
 \label{fig:3SAOSSweep}
 \end{figure}
 
 \begin{figure}[h!]
 \includegraphics{Figures/Chapter3/FigMAOSCP-radj.pdf}%
 \caption{First-ever MAOStress material functions measurement as a function of frequency. The normalized intrinsic first-harmonic (a) elastic $[c_1]/J_0^3$and (b) viscous $[f_1]/\phi_0 J_0^2$ MAOStress material functions show that PVA-Borax stiffens and thickens under weakly-nonlinear stress forcing. The normalized intrinsic third harmonic (a) elastic $[c_3]/J_0^3$and (b) viscous $[f_3]/\phi_0 J_0^2$ MAOStress material functions tell the reason behind the observed stiffening and thickening. Open symbols represent negative values, and closed symbols represent positive values. \label{fig:3MAOSsweep}}%
 \end{figure}
 
The choice of normalization in Figure \ref{fig:3MAOSsweep} was based on the scaling observed in the Strain-Stiffening Transient Network Model (SSTNM) and the time-strain separable MAOS model. Even though they are independent, the linear and nonlinear MAOStress material functions may scale with a measure of the linear elastic compliance $J_0$ or fluidity $\phi_0$. Similar behavior is observed in MAOStrain, where for many constitutive models, the linear and nonlinear material functions scale with $G_0$ and $\eta_0$. These scalings emerge from the physics that underlies the behavior of the material. While no model is correct, they can still capture essential aspects of the material physics reflected in the predicted scaling. The SSTNM model was developed by Bharadwaj et al. in 2017 to model the strain-stiffening MAOS behavior of PVA-Borax, where none of the existing nonlinear viscoelastic models was able to capture the behavior of this material\cite{Bharadwaj2017AShear}. Solving the SSTNM model numerically in stress control mode (Check Appendix B) yields the normalization used in Figure \ref{fig:3MAOSsweep}. The results were corroborated by applying the Lennon et al.\cite{Lennon2020MediumExamples} interrelations to the analytical solution\cite{Bharadwaj2017AShear} of the MAOStrain material functions of the SSTNM model.
Moreover, applying the same relations to the time-strain separable MAOS models with a single-mode relaxation kernel yields the same scaling relationship. The MAOS time-strain separable (TSS) models are a generic category for which time-strain separability holds and where the damping function is expanded up to only the first deviation from linearity\cite{Martinetti2019Time-strainShear}. These findings suggest that the chosen normalization is suitable for comparing data from different materials as it provides a measure of nonlinearity independent from the linear compliance and fluidity for various models of nonlinear viscoelasticity.

%The main goal of the normalization is to report a measure of the relative nonlinearity strength with respect to the linear component. This reduction will ensure that the magnitude of the reported nonlinearity can be compared between different  materials that may have a different absolute linear compliance or modulus.

Other choices of normalization can be derived by examining Eqn~\ref{eq:3 harmnonics expansion} but will have different physical interpretations as summarized in Table~\ref{Tab:Interpret}. The unnormalized material functions (e.g., $[c_1]$) quantify the rate at which the absolute nonlinear deviation (e.g., $[c_1]\sigma_0^3$) grows per unit of $\sigma_0^3$. However, when comparing different materials, the ratio of the deviation (e.g., $[c_1]\sigma_0^3$) to the linear term (e.g., $J_1^{\prime}\sigma_0$) is more relevant. Therefore, another choice to normalize $[c_1]$ is $\frac{[c_1]}{J^{\prime}}(\omega)$ (similar normalization for the other material functions shown in Table~\ref{Tab:Interpret}), which quantifies the rate at which the magnitude of the ratio $\frac{[c_1]\sigma_0^3}{J_1^{\prime}\sigma_0}$ grows per unit of $\sigma_0^2$. Moreover, the ratio $\frac{[c_1]\sigma_0^2}{J_1^{\prime}}$ justifies the scaling inferred from the SSTNM and MAOS TSS models, e.g.$[c_1]$ scales with $J_0^3$.  For a single-mode SSTNM model, $J^{\prime}(\omega)=J_0$, and the stress amplitude is to first-order proportional to $G_0=1/J_0$ for any particular strain. Hence, $[c_1]/J_0^3$ can be interpreted as the relative nonlinearity $\frac{[c_1]\sigma_0^3}{J^{\prime}\sigma_0}$ at a comparable measure of strain ($\gamma \approx \sigma_0 J^{\prime}= \sigma_0 J_0=1$ in this case). This reasoning indicates that for the SSTNM and MAOS TSS models, the relative nonlinearity is constant for the same nonlinear parameter ($\alpha$ or $A$, respectively, as defined in the SI) when different materials are compared at equivalent strains, which is consistent with the fact that the accumulated strain in these models sets the degree of nonlinearity. Since PVA-Borax cannot be described by a single-mode relaxation model, $J_0$ can be replaced with $J^{\prime}$ and $\phi_0$ with $\phi^{\prime}$ to have the same interpretation at different frequencies. Comparing the frequency dependence of $\frac{[c_1]}{J_0^3}$ and $\frac{[c_1]}{J^{\prime 3}}$ in Figure \ref{fig:3MAOSsweepnorm2} shows that the latter normalization varies less with frequency achieving a constant plateau for $\omega>0.3$ rad/s. This observation shows that incorporating the frequency dependence of the linear material functions in the normalization helps reduce the complexity of the material behavior, which shows a near-constant relative nonlinearity as a function of frequency. 
% Please add the following required packages to your document preamble:

\begin{table}
\caption{Normalization choices for MAOStress intrinsic nonlinearities. Frequency dependence is implied for all variables except the constants $J_0$ and $\phi_0$. 
 \label{Tab:Interpret}}
\begin{center}
\renewcommand\arraystretch{1.2}
\begin{tabular}{| >{\raggedright\arraybackslash}p{0.33\linewidth} | >{\raggedright\arraybackslash}p{0.33\linewidth} |>{\raggedright\arraybackslash}p{0.33\linewidth}|}
\hline
\textbf{Type} & \textbf{Material Functions} & \textbf{Comments} \\ \hline
Absolute nonlinearities &        $[c_1]$, $[f_1]$, $[c_3]$, and $[f_3]$            &        Rate of growth of harmonic deviation per $\sigma_0^3$   \\ \hline
   Relative nonlinearities  &        $\frac{[c_1]}{J^{\prime}}$, $\frac{[f_1]}{\phi^{\prime\prime}}$, $\frac{[c_3]}{J^{\prime}}$, and $\frac{[f_3]}{\phi^{\prime\prime}}$            &   Rate of growth of relative harmonic deviation per $\sigma_0^2$          \\\hline
Model-informed normalized nonlinearity (Single-mode)& $\frac{[c_1]}{J_0^3}$, $\frac{[f_1]}{J^2_0 \phi_0}$, $\frac{[c_3]}{J_0^3}$, and $\frac{[f_3]}{J^2_0 \phi_0}$    & Dimensionless. Quantifies relative nonlinearity at $\gamma \approx J_0\sigma_0= 1$    \\ \hline
  Model-informed normalized nonlinearity (Multi-mode)& $\frac{[c_1]}{J^{\prime 3}}$, $\frac{[f_1]}{J^{\prime 2} \phi^{\prime}}$, $\frac{[c_3]}{J^{\prime 3}}$, and $\frac{[f_3]}{J^{\prime 2} \phi^{\prime}}$    & Accounts for multi-mode relaxation (varying $J^{\prime}(\omega)$ and $\phi^{\prime}(\omega)$) 
\\ \hline

\end{tabular}

\end{center}
 
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}


\section{Discussion}
\label{Sec:3Discuss}
One of the interesting features to discuss in the frequency dependent linearity limits $\sigma_{crit}(\omega)$, $\gamma_{crit}(\omega)$, and $\dot{\gamma}_{crit}(\omega)$, what can be used as regime boundaries in Pipkin maps.The Pipkin map was initially proposed in 1972 as a tool to map the behavior of complex fluids based on two dimensions: frequency (inverse timescale) and amplitude \cite{Pipkin1986LecturesTheory}. This map has proven to be a valuable means of comparing the behavior of complex fluids under comparable conditions. Notably, Pipkin did not specify a particular measure of nonlinearity, leaving it open for interpretation. Commonly used measures include strain amplitude and the strain-rate amplitude (or Weissenberg number, sometimes written as Wi$\equiv \dot{\gamma\tau}$)\cite{Macosko1994Rheology:Applications,Dealy1999MeltProcessing,Ewoldt2013Low-dimensionalViscoelasticity,Giacomin2011Large-amplitudeModel}. In the case of strain amplitude, the linearity limit line exhibits a critical strain that diverges as the Deborah number (De) approaches zero. Conversely, when using strain rate or the Weissenberg number, the linearity limit line approaches a constant value in the elastic limit and diverges to infinity in the viscous limit. The frequency dependence of the linearity limit based on stress has not been previously predicted or measured, and MAOS offers an effective means of experimental and numerical exploration.

\subsection{Defining a threshold-independent critical forcing amplitude}
Ewoldt and Bharadwaj used MAOS material functions as a rigorous way to define linearity limit lines \cite{Ewoldt2013Low-dimensionalViscoelasticity}. Since the emergence of nonlinearities is grdual, the choice of where the linear regime ends is arbitrary and depends on a specified threshold $\epsilon$. Relying on visually perceived plateaus prevents consistent comparison of linearity limits. MAOS material functions can directly compare the weakly nonlinear terms in the expansion to linear terms, providing a quantitative measure of the critical value (strain, strain-rate, or stress) independent of the chosen threshold. This approach was used for MAOStrain, where the critical strain $\gamma_{crit}$ for nonlinearity was defined as the strain where the ratio of the weakly nonlinear deviation of the stress harmonics to the linear term exceeds a set threshold. However, it was applied to model solutions and not experimental data. Pearson and Rochehfort did the first experimental measurement of a critical strain from oscillatory measurements in 1982\cite{Pearson1982BehaviorFields}, where they defined the elastic critical strain at $\big|\frac{G^{\prime}_{13}-G^{\prime}_{11}}{G^{\prime}_{11}}\big|=5\%$ and the viscous critical strain at $\big|\frac{G^{\prime\prime}_{13}-G^{\prime\prime}_{11}}{G^{\prime\prime}_{11}}\big|=5\%$.  Here, we use the MAOStress material functions to compute the critical stress to go nonlinear $\sigma_{crit}$ based on the four independent material functions. Setting the ratio of the elastic and viscous weakly nonlinear deviations $[c_1]\sigma_0^3$ and $\frac{[f_1]}{\omega}\sigma_0^3$ to the corresponding linear terms $J^{\prime}\sigma_0$ and $J^{\prime\prime}\sigma_0$ to the threshold $\epsilon$, we can define critical stress based on the first-harmonic nonlinearities as:
%To Think: Why are we comparing third harmonics to only one linear component? Is there a reasoning? Should be the total magnitude probably. 
\begin{subequations}
\label{eq:3critStressFirstHarmonics}
\begin{eqnarray}
\frac{[c_1]\sigma_{crit}^3}{J^{\prime}\sigma_{crit}}= \epsilon \qquad \Rightarrow \qquad \frac{\sigma_{crit,[c_1]}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{ J^{\prime}}{[c_1]}}\\
\frac{[f_1]\sigma_{crit}^3}{J^{\prime\prime}\omega\sigma_{crit}}=\epsilon \qquad \Rightarrow \qquad \frac{\sigma_{crit,[f_1]}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{ \phi^{\prime}}{[f_1]}}
\end{eqnarray}
\end{subequations}
Similarly, for the third harmonics, we set the ratio of the elastic and viscous weakly nonlinear deviations $[c_3]\sigma_0^3$ and $\frac{[f_3]}{3 \omega}\sigma_0^3$ to the corresponding linear terms $J^{\prime}\sigma_0$ and $J^{\prime\prime}\sigma_0$ to the threshold $\epsilon$ to obtain:
\begin{subequations}
\label{eq:3critStressThirdHarmonics}
\begin{eqnarray}
\frac{[c_3]\sigma_{crit}^3}{J^{\prime}\sigma_{crit}}=\epsilon \qquad &\Rightarrow \qquad \frac{\sigma_{crit,[c_3]}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{ J^{\prime}}{[c_3]}}\\
\frac{[f_3]\sigma_{crit}^3}{3 J^{\prime\prime}\omega\sigma_{crit}}=\epsilon \qquad &\Rightarrow  \qquad \frac{\sigma_{crit,[f_3]}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{3  \phi^{\prime}}{[f_3]}}
\end{eqnarray}
\end{subequations}
Eqns. \ref{eq:3critStrainFirstHarmonics} and \ref{eq:3critStrainThirdHarmonics} reveal that a threshold-independent critical stress can be reported, which will make the comparison of different results easier. This applies to others measures of nonlinearity such as strain and strain rate. We recommend future works to report critical forcing amplitudes as follows
$$\frac{\sigma_{crit}}{\sqrt{\epsilon}},\;\frac{\gamma_{crit}}{\sqrt{\epsilon}}\;\frac{\dot{\gamma}_{crit}}{\sqrt{\epsilon}}.$$
This approach allows for better comparison of critical forcing amplitudes, but we acknowledge that it strictly applies for small enough forcing amplitudes/chosen threshold, where the higher order terms can be neglected. 

Figure \ref{fig:3critStressExpAll} shows how each critical stress depends on Deborah number $\mathrm{De}$ by applying Eqs. 10-11 to the data in Figure \ref{fig:3MAOSsweep}. These lines represent the boundaries between the linear and weakly nonlinear regimes on a Pipkin map constructed using stress to measure the nonlinearity strength. The results show that the first-harmonics are the first to reach a nonlinearity threshold, also observed in the amplitude sweeps shown in Figure \ref{fig:3AmpSweep}. Moreover, the first harmonics have a weak frequency dependence compared to those exhibited by strain and strain rate first harmonics, as shown in Figure \ref{fig:3MAOStrainFirstAndThird}. A peak occurs at 10 rad/s for the third harmonics, concurrent with the sign change in $[c_3]$ and drop in $[f_3]$. The results in Figure \ref{fig:3critStressExpAll} reveal that the MAOStress behavior of this PVA-Borax formulation was accessible because the stress required to measure the nonlinear material functions was in an accessible range that did not cause irreversible changes to the material. This allowed multiple frequencies to be tested per loading, simplifying the experimental procedure. %The presence of these peaks highlights how using one nonlinear signal is insufficient to define a critical stress; instead, all the signals should be considered. 
%Comparing the frequency dependence of the critical stress to the critical strain and strain rate is more straightforward if one critical value is defined for each.  Below, we propose an approach to compare the Pipkin diagram boundary between the linear and nonlinear regimes for $\sigma$, $\gamma$, and $\dot{\gamma}$.

\begin{figure}[h!]
\centering
 \includegraphics{Figures/Chapter3/CriticalStressExperimental1.0Radj.pdf}%
 \caption{Critical stress for the weakly nonlinear transition. The critical stress to enter the nonlinear regime was computed based on each of the MAOStress material functions, reported in Figure \ref{fig:3MAOSsweep}, using Eqs. \ref{eq:3critStressFirstHarmonics}(a-b) and \ref{eq:3critStressThirdHarmonics}(a-b). The elastic (red) and viscous (blue) material functions reveal comparable critical stress for the first harmonics but differ slightly for the third harmonics.    \label{fig:3critStressExpAll}}%
 \end{figure}

\subsection{Pipkin Map linearity limits: Stress, Strain, or Strain-rate}
This section will compare the Pipkin map regime boundary of the linear regime when either stress, strain, or strain rate is considered. We derived a single critical stress instead of four values from the different material functions to facilitate this. One viable approach is to choose the minimum of the four independent critical stresses defined in Eqs.~\ref{eq:3critStressFirstHarmonics} and ~\ref{eq:3critStressThirdHarmonics}.  The drawback of this approach is that the critical stress linearity limit line will be noisy as the criteria shift between different metrics. To resolve this issue, we define a single critical stress based on the first harmonics by finding the stress at which the magnitude of the total first-harmonic deviation exceeds a threshold in comparison to the magnitude of the linear first-harmonic modulus
\begin{subequations}
\label{eq:3pipkinLimitsMAOStressFirst}
\begin{eqnarray}
\frac{\sqrt{([c_1]\sigma_{crit}^3)^2+(\frac{[f_1]}{\omega}\sigma_{crit}^3)^2}}{\sqrt{(J^{\prime}\sigma_{crit})^2+(J^{\prime\prime}\sigma_{crit})^2}}=\epsilon \qquad \Rightarrow \qquad \frac{\sigma_{crit,1}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{|J^{*}|}{\sqrt{([c_1])^2+\left(\frac{[f_1]}{\omega}\right)^2}}}.
\end{eqnarray}
\end{subequations}
$\sigma_{crit,1}$ is the stress at which the first-harmonic deviations affect both the observed elastic and viscous Lissajous curves, particularly in terms of the rotation and enclosed area. Moreover, we define $\sigma_{crit,3}$ as the critical stress at which the magnitude of the total third harmonic deviation exceeds a threshold with respect to the magnitude of the linear viscoelastic
\begin{subequations}
\label{eq:3pipkinLimitsMAOStressThird}
\begin{eqnarray}
\frac{\sqrt{([c_3]\sigma_{crit}^3)^2+(\frac{[f_3]}{3\omega}\sigma_{crit}^3)^2}}{\sqrt{(J^{\prime}\sigma_{crit})^2+(J^{\prime\prime}\sigma_{crit})^2}}=\epsilon  \qquad \Rightarrow \qquad  \frac{\sigma_{crit,3}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{ |J^{*}|}{\sqrt{([c_3])^2+\left(\frac{[f_3]}{3\omega}\right)^2}}}.
\end{eqnarray}
\end{subequations}
$\sigma_{crit,3}$ is the stress at which the third-harmonic deviations affect both the observed elastic and viscous Lissajous curves, particularly in terms of the distortion from their linear elliptical shape. Finally we define $\sigma_{crit}$ as the minimum of $\sigma_{crit,1}$ and $\sigma_{crit,3}$:

\begin{equation}
    \sigma_{crit}=\mathrm{min}(\sigma_{crit,1},\sigma_{crit,3})
    \label{Eq:3criticalStressFinal}
\end{equation}

Similarly, the critical strain for nonlinearity can be computed from the MAOStrain material functions, measured on the ARES-G2 rheometer as described in Appendix C. The critical strain $\gamma_{crit}$ is the minimum of $\gamma_{crit,1}$ and $\gamma_{crit,3}$
\begin{equation}
        \gamma_{crit}=\mathrm{min}(\gamma_{crit,1},\gamma_{crit,3})
    \label{Eq:3criticalStrainFinal}
\end{equation}
which are defined as
\begin{subequations}
\label{eq:3critStrainFirstHarmonics}
\begin{eqnarray}
\frac{\sqrt{([e_1]\gamma_{crit}^3)^2+([\omega v_1]\gamma_{crit}^3)^2}}{\sqrt{(G^{\prime}\sigma_{crit})^2+(G^{\prime\prime}\sigma_{crit})^2}}=\epsilon \qquad \Rightarrow \qquad \frac{\gamma_{crit,1}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{ |G^{*}|}{\sqrt{([e_1])^2+(\omega[v_1])^2}}},
\end{eqnarray}
\end{subequations}
and
\begin{subequations}
\label{eq:3critStrainThirdHarmonics}
\begin{eqnarray}
\frac{\sqrt{([e_3]\gamma_{crit}^3)^2+([\omega v_3]\gamma_{crit}^3)^2}}{\sqrt{(G^{\prime}\sigma_{crit})^2+(G^{\prime\prime}\sigma_{crit})^2}}=\epsilon\qquad  \Rightarrow \qquad  \frac{\gamma_{crit,3}(\omega)}{\sqrt{\epsilon}}=\sqrt{\frac{ |G^{*}|}{\sqrt{([e_3])^2+(\omega[v_3])^2}}}.
\end{eqnarray}
\end{subequations}
The critical strain-rate amplitude can be obtained from the critical strain as \begin{equation}
    \dot{\gamma}_{crit}=\gamma_{crit}\omega
\end{equation}
Figure \ref{fig:3pipkinMapExp} compares the critical stress, strain, and strain rate, all normalized to be dimensionless. Remarkably, the normalized stress approaches the critical strain in the elastic limit (high Deborah number) and the normalized critical strain rate in the viscous limit (low Deborah number). This result can be justified because the stress is dominated by the viscous contribution at low frequencies and elastic effects at high frequencies for any viscoelastic liquid material. For PVA-Borax, the nonlinearity is related to local stretch of the polymer chains in the transient polymer network\cite{Bharadwaj2017AShear,Martinetti2018InferringNetwork}. The network will behave elastically at time-scales shorter than the time-scale of bond dissociation. At those timescale ($De\to \infty$), the strain applied is fully translated into stretch of the polymer strands, which will exceed the linearity threshold at a critical characteristic strain $\gamma_{crit}$, consistent with the physical picture. This critical strain is equivalent to a critical stress $\sigma_{crit}=G_0 \gamma_{crit}$, as all the stress would come from the elastic deformation. In the viscous limit ($De \to 0$), the network will quickly relax the stress from the applied strain and the polymer stretch will be proportional to the applied strain rate $\propto \dot{\gamma}\tau$ (equivalent to a Weissenber number\cite{White1964DynamicsSpinning}), where $\tau$ is a characteristic timescale. Therefore, the critical strain rate $\gamma_{crit}$ for nonlinearity will be constant in that limit and will be determined by the degree of stretch required in the polymer strands. The stress in this limit will also be constant and will be equal to $\sigma_{crit}=\eta_0\dot{\gamma}_{crit}=G_0\tau_C\dot{\gamma}_{crit}$. Therefore, as long as the characteristic timescale $\tau$ that determines the stretch in polymer strands is close to the average relaxation time $\tau_C$, the critical stress in the elastic limit and viscous limit will be equivalent. However, if these two timescales differ (e.g. polydisperse systems), the critical stress may be different. 

The universality of critical stress is also expected to hold more generally to all viscoelastic liquids. Any viscoelastic liquid is expected to have a constant critical strain $\gamma_{crit}$ in the elastic limit ($De\to\infty$) and a constant critical strain rate $\dot{\gamma}_{crit}$ in the viscous limit ($De \to \infty$). Therefore, the critical stress ($\sigma_{crit}= G_0\gamma_{crit}$ for De>>1 and $\sigma_{crit}= \eta_0 \dot{\gamma}_{crit}$ for De<<1) will be constant in each of these limits. In contrast to critical stress, the critical strain and strain rate will always have a diverging behavior at one of the limits for any viscoelastic liquid. Therefore, critical stress is expected to be a more universal measure of nonlinearity strength, as observed here experimentally. 

The universality of critical stress may allow for faster characterization of material properties using the frequency-sweep MAOS method\cite{Singh2017Frequency-sweepMAOS}. This technique eliminates the need for a full amplitude sweep at every frequency and instead relies on the ability to predict at which amplitude the MAOS material functions can be measured. Based on that prediction, a single amplitude measurement is done at every frequency. Since the critical stress varies slightly as a function of De compared to critical strain, applying the frequency-sweep MAOS technique in MAOStress should be simpler. This will result in a high-throughput characterization while minimizing the impact of chemical and physical changes in the loaded material. Additionally, this work shows that the change in the critical stress amplitude required to measure MAOStress nonlinearities is much smaller than MAOStrain measurements, making the MAOStress technique potentially more accessible than MAOStrain. 

 \begin{figure}[h!]
 \centering
 \includegraphics{Figures/Chapter3/Fig7PipkinMapCompareExp.pdf}%
 \caption{Comparing Pipkin Diagram nonlinear transition limits. Normalized critical stress, strain, and strain rate values estimated from MAOStrain (Eq.\ref{Eq:3criticalStressFinal})and MAOStress (Eq.\ref{Eq:3criticalStrainFinal}) material functions (Figures \ref{fig:3SAOSSweep} and \ref{fig:3MAOSsweep}) obtained experimentally for PVA-Borax 1.25/2.75 wt\%. The critical stress appears to be a more universal measure of nonlinearity as a function of frequency, where it varies between the finite critical strain rate and strain limits at low and high De, respectively.   \label{fig:3pipkinMapExp}}%
 \end{figure}
\section{Conclusion}
The MAOStress response of PVA-Borax was thoroughly studied, showing that stress-controlled measurements can offer another route for testing the weakly nonlinear regime and answer fundamental questions regarding the origins of nonlinearity in viscoelastic materials. The MAOStress results confirmed the stiffening nature of PVA-Borax and showed that stress is a more universal measure of nonlinearity strength across a wide range of De, consistent with the microstructure of PVA-Borax. Moreover, the measured linearity limits can be interpreted as Pipkin map regime boundaries, offering experimental testing and validation of theoretical predictions. The SSTNM model was used to derive a viable normalization of the nonlinear MAOStress material functions that account for their scaling with the linear material properties. The frequency dependence of the normalized material functions revealed a simplicity in the features of MAOStress material functions compared to MAOStrain. This simplicity could be harnessed in future works that compare MAOStress measurements with model predictions for physical inference.

The intrinsic nonlinearities were used to show that stress is a more universal measure of nonlinearity strength as its frequency variability at the emergence of nonlinearity is much smaller than MAOStrain. This fundamental result should be considered when studying deformation-induced physical phenomena at different timescales or frequencies. Moreover, this result has significant implications for small amplitude oscillatory shear measurements (SAOS). A common practice for choosing a strain or stress amplitude for a linear SAOS measurement is to do an amplitude sweep at different frequencies and choose a strain or stress in different frequency ranges with a good signal-to-noise ratio without being in the nonlinear regime. With the insights from section IV, it may suffice to only do an amplitude sweep at each end of the frequency range to find a suitable stress amplitude for the entire frequency range of a measurement. 

The findings of this work motivate future exploration of the MAOStress response of other materials. For example, comparing the MAOStress material functions of multiple PVA-Borax formulations could be very insightful in understanding the effect of microstructural changes on the material properties. Moreover, testing different viscoelastic materials, such melts, colloids, and multicomponent systems, will also highlight the effect of the microstructure on the MAOStress response.

\section*{Acknowledgements}
This work was funded by the U.S. Department of Energy, Office of Basic Energy Sciences, Division of Materials Sciences and Engineering under Award DE-SC0020858, through the Materials Research Laboratory at the University of Illinois at Urbana-Champaign. The authors are grateful to Anton Paar for loaning the MCR 702 instrument to the Ewoldt Research Group, which enabled the MAOStress measurements.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
